A Multi-Epoch Study of Radio Continuum Emission from MassiveProtostars

We report the results of the Jansky Very Large Array (JVLA) observation of five massive protostars at 6 and 22.2 GHz. The aim of the study was to compare their current fluxes and positions with previous observations to search for evidence of variability. Most of the observed sources present the morphologies of a thermal core, hosting the protostar and exhibiting no proper motion, and associated non-thermal radio lobes that are characterised by proper motions and located away from the thermal core. Some of the protostars drive jets whose lobes have dissimilar displacement vectors, implying precession of the jets or the presence of multiple jet drivers. The jets of the protostars were found to have proper motions that lie in the range 170$ \leq v \leq $650 kms$^{-1}$, and precessions of periods 40$\leq p \leq$50 years and angles 2$\leq \alpha \leq$10$^\circ$, assuming that their velocities $v=$500 kms$^{-1}$. The core of one of the sources, S255 NIRS 3, which was in outburst at the time of our observations, showed a significant change in flux compared to the other sources. Its spectral index decreased during the outburst, consistent with the model of an expanding gas bubble. Modelling the emission of the outburst as that of a new non-thermal lobe that is emerging from a thermal core whose emission enshrouds that of the lobe also has the potential to account for the increase in flux and a decrease in the spectral index of the source's outburst.

==> README <==
% readme.txt
%
% MNRAS journal LaTeX package
% v3.0 for LaTeX 2e
%
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `author-maintained'.
% 
% The Current Maintainer of this work is: Royal Astronomical Society,
% MNRAS Editorial Office, who can be contacted on mn@ras.org.uk
%
% This work consists of all the files listed in readme.txt
%
%
% Last updated 22 May 2015
%
% Copyright (C) Royal Astronomical Society 2015, Blackwell Science 2001,
% Cambridge University Press 1994
%
% See each file for a detailed author list and change log.
%
% This package consists of the following files:

readme.txt          This file

mnras.cls           MNRAS LaTeX document class
mnras.bst           MNRAS BibTeX style

mnras_guide.tex     User guide, LaTeX format
mnras_guide.pdf     User guide, PDF format
mnras_template.tex  A simple template paper

example.eps         An example image used in the guide
example.png         An example image used in the guide
example.ps          An example image used in the guide

legacy\legacy.txt   Description of the legacy releases
legacy\mn2e.cls     v2.2 of mn2e.cls (deprecated)
legacy\mn2e.bst     v1.1b of mn2e.bst (deprecated)


% Disclaimer:
%
% This LaTeX package is provided free to the community in the hope that it
% assists them in preparing papers for the journal Monthly Notices of the
% Royal Astronomical Society.
% The files are provided 'as-is' with no guarantee of their suitability,
% freedom from errors or omissions, or compatibility with any software.
% The Royal Astronomical Society cannot provide user support for this package,
% LaTeX, or for any other software.
% Authors are free to use other styles or programmes if they wish.
% Please see the journal instructions to authors for guidance.
% This disclaimer is in addition to the No Warranty section of the licence,
% at the link given above.
